Modelling of highly extended Gamma-ray emission around the Geminga Pulsar as detected with H.E.S.S

Geminga is an enigmatic radio-quiet gamma-ray pulsar located at a mere 250 pc distance from Earth. Extended very-high-energy gamma-ray emission around the pulsar has been detected by multiple water Cherenkov detector based instruments. However, the detection of extended TeV gamma-ray emission around the Geminga pulsar has proven challenging for IACTs due to the angular scale exceeding the typical field-of-view. By detailed studies of background estimation techniques and characterising systematic effects, a detection of highly extended TeV gamma-ray emission could be confirmed by the H.E.S.S. IACT array. Building on the previously announced detection, in this contribution we further characterise the emission and apply an electron diffusion model to the combined gamma-ray data from the H.E.S.S. and HAWC experiments, as well as X-ray data from XMM-Newton.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

